$BT^2$: Backward-compatible Training with Basis Transformation

Modern retrieval system often requires recomputing the representation of every piece of data in the gallery when updating to a better representation model. This process is known as backfilling and can be especially costly in the real world where the gallery often contains billions of samples. Recently, researchers have proposed the idea of Backward Compatible Training (BCT) where the new representation model can be trained with an auxiliary loss to make it backward compatible with the old representation. In this way, the new representation can be directly compared with the old representation, in principle avoiding the need for any backfilling. However, followup work shows that there is an inherent tradeoff where a backward compatible representation model cannot simultaneously maintain the performance of the new model itself. This paper reports our ``not-so-surprising'' finding that adding extra dimensions to the representation can help here. However, we also found that naively increasing the dimension of the representation did not work. To deal with this, we propose Backward-compatible Training with a novel Basis Transformation ($BT^2$). A basis transformation (BT) is basically a learnable set of parameters that applies an orthonormal transformation. Such a transformation possesses an important property whereby the original information contained in its input is retained in its output. We show in this paper how a BT can be utilized to add only the necessary amount of additional dimensions. We empirically verify the advantage of $BT^2$ over other state-of-the-art methods in a wide range of settings. We then further extend $BT^2$ to other challenging yet more practical settings, including significant change in model architecture (CNN to Transformers), modality change, and even a series of updates in the model architecture mimicking the evolution of deep learning models.

==> CVPR_submission/exps.tex <==
\section{Experiments}
\label{sec:experiments}
Our experiments are designed to verify (1) whether existing backward compatible representation learning methods can achieve satisfying performances in terms of achieving reliable backward compatibility and not hurting the new model in practice, (2) whether our proposed method can provide reliable empirical strength extending to extremely diverse backward compatible cases such as open classes, significant changes in model architecture (for example, ResNet to pretrained Transformers), different modalities, and a series changes of model architecture (mimicing the historical development), and (3) how does varying the number of extra dimensions change the performance of our methodology.

\subsection{Datasets}
This work makes use of the following datasets:
\begin{itemize}
    \item \emph{Cifar-100}\cite{cifar100}: Cifar-100 is a popular image classification dataset consisting of 60000 images in 100 classes. We use Cifar-50 to refer the partition consisting of all the images from the first 50 classes.
    
    \item \emph{Imagenet-1k} \cite{5206848}: Imagenet-1k is a large-scale image recognition dataset for ILSVRC 2012 challenge. It has 1000 image classes with approximately 1.2k images per class. We follow the same partition as \cite{ramanujan2022forward} where we use the images from the first 500 classes as Imagenet-500.
\end{itemize}
\subsection{Evaluation Metrics}
We follow the standard notation and evaluation metrics used by \cite{9156906, ramanujan2022forward}. We use the notation Query Embedding/Gallery Embedding to denote which model we are using for query and gallery embedding respectively. For example, $\phi_{new}/\phi_{old}$ refers to using the new model for the query embedding and the old model for the gallery embed- ding. The evaluation task (retrieval from the gallery set) is fixed, while the old and new embedding models are trained differently.

\paragraph{Cumulative Matching Characteristics (CMC)} corresponds to the top-k accuracy, where we sort the gallery representations by their similarity to the query representation. It is considered correct if a match with the same class is in the first k gallery representations. We report CMC top-1 and top-5 for all models. 

\paragraph{Mean Average Precision (mAP)} is a standard metrics that summarizes precision and recall metrics by taking the area under the precision-recall curve. We compute the avergae precision in the recall value in [0.0, 1.0].

\subsection{Baselines}
We adopt the following baselines to validate our results.
\paragraph{Backward Compatible Training (BCT)} is adopted from Shen \etal \cite{9156906}. Although it was the first attempt for backward compatibility, it is still frequently adopted as a strong baseline in many recent papers\cite{ramanujan2022forward, https://doi.org/10.48550/arxiv.2204.13919}. Specifically, they adopt classification to train the representation loss. BCT adds a designed "influence loss" to the training of the new model, so that it can bias the new representation model towards the one that can be used compatible with the old classifier. Denote $w_{\phi}$ is the new representation model, $w^c$ is a trainable classification head, while $w^c_{old}$ is the fixed classification head that was trained with the old representation head. They adopt the following combined loss to train a backward compatible new representation model:
\begin{align*}
    \mathcal{L}_{BCT} = \mathcal{L}(w^c, w_{\phi}) + \lambda \mathcal{L}(w^c_{old}, w_{\phi}),
\end{align*}
where $\lambda$ is a hyperparameter to tune, $\mathcal{L}(w^c, w_{\phi})$ represents a classification loss with $w^c$ as the classification head and $w_{\phi}$ as the representation, and so is $\mathcal{L}(w^c, w_{\phi})$.
\paragraph{Backward Compatible Training with 32 Extra Dimension (BCT(+32))}. We hypothesize that adding new dimensions might also be helpful for BCT. Therefore, to make it a fair comparison with our method, where we adds 32 dimensions compared to BCT, we also make this variant to BCT where we allows the new representation to have a dimension expansion of 32. We use the same loss function as BCT except that we pad the missing dimension of $w^c_{old}$ with 0.

\paragraph{Regression-alleviating Compatibility Regularization (contrast)} is a recently proposed more sophisticated auxiliary loss for backward compatiblility \cite{DBLP:journals/corr/abs-2201-09724}. The influence loss in BCT is replaced with the following loss:

\begin{align*}
    &\mathcal{L}_{ra-comp}(x) =\\
    & \log (1 + \frac{\sum_{k \in \mathcal{B} - p(x)}\exp{\phi_{new}(k) \cdot \phi_{old}(k)/\tau}}{\exp{\phi_{new}(x) \cdot \phi_{old}(x)/\tau}}\\
    +& \frac{\sum_{k \in \mathcal{B} - p(x)} \exp{\phi_{new}(k) \cdot \phi_{new}(k)/\tau}}{\exp{\phi_{new}(x) \cdot \phi_{old}(x)/\tau}}),
\end{align*}
where $\mathcal{B}$ is the mini-batch for training, $p(x)$ is the set of samples in the minibatch with the same label as $x$, and $\tau$ is a hyperparameter of temperature.

\paragraph{BCT-BX (ours)} is the instantiation of our methodology described in Section \ref{sec:merge} with the allowed dimension expansion to be 32. We use classification loss for the mimicing $\phi_{new}'$, and a combination of cosine similarity loss and influence loss for mimicing $\phi_{old}'$.

\subsection{Notes on Using Cosine Similarity or Euclidean Distance}
We do want to note that some of the previous works on representation learning use Euclidean Distance as a similarity for retrieval \cite{9156906, ramanujan2022forward} while others use Cosine Similarity as a similarity measure \cite{DBLP:journals/corr/abs-2108-01958, DBLP:journals/corr/abs-1904-06627, DBLP:journals/corr/abs-2006-07733, DBLP:journals/corr/abs-2003-08505, DBLP:journals/corr/abs-2103-00020}. In our preliminary experiments compared with public results in \cite{9156906, ramanujan2022forward} , we did not find 
clear superiority of any of the similarity measure. We therefore adopt cosine similarity for a clearer analysis and better compatibility with our experiments on multi-modality.
\subsection{Data Change}

\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ c c c c }
\hline 
\multirow{2}{5em}{Method} & \multirow{2}{3em}{Case} & CMC & \multirow{2}{5em}{mAP@1.0} \\
& & top1-top5 &\\
\hline
\multirow{3}{5em}{Independent} & $\phi_{old}/\phi_{old}$ & 33.6-55.4 & 24.4\\
& $\phi_{new}'/\phi_{old}$ & 0.8-4.9 & 1.5\\
& $\phi_{new}'/\phi_{new}'$ & 62.7-74.6 & 49.9\\
\hline
\multirow{2}{5em}{BCT} & $\phi_{new}^{bct}/\phi_{old}$  & 23.5-60.4 & 23.9\\
& $\phi_{new}^{bct}/\phi_{new}^{bct}$ & 56.1-70.8 & 43.6\\
\hline
\multirow{2}{5em}{BCT (+32)} & $\phi_{new}^{bct(+32)}/\phi_{old}$ & 22.1-61.3& 23.8\\
& $\phi_{new}^{bct(+32)}/\phi_{new}^{bct(+32)}$ & 56.1-71.3 & 44.1\\
\hline
\multirow{2}{5em}{contrast} & $\phi_{new}^{contrast}/\phi_{old}$ & 26.1-61.8 & 25.1\\
& $\phi_{new}^{contrast}/\phi_{new}^{contrast}$ & 57.9-75.2 & 36.7\\
\hline
\multirow{2}{5em}{BCT-BX (Ours)} & $\phi_{new}^{bct-bx}/\phi_{old}$ & \textbf{43.3}-\textbf{68.7} & \textbf{27.7}\\
& $\phi_{new}^{bct-bx}/\phi_{new}^{bct-bx}$ & \textbf{64.2}-\textbf{77.0} & \textbf{53.1}\\
\hline
\end{tabular}}
\caption{Backward compatible experiments on cifar-50 to cifar-100 with only data change. Both the old model and the new model uses Resnet50-128 architecure.}
\label{table:cifar100 data change}
\end{center}
\end{table}

\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ c c c c }
\hline 
\multirow{2}{5em}{Method} & \multirow{2}{3em}{Case} & CMC & \multirow{2}{5em}{mAP@1.0} \\
& & top1-top5 &\\
\hline
\multirow{3}{5em}{Independent} & $\phi_{old}/\phi_{old}$ & 43.1-58.3 & 30.9\\
& $\phi_{new}'/\phi_{old}$ &0.1-0.5  & 0.2\\
& $\phi_{new}'/\phi_{new}'$ & 67.9-81.4 & 52.3\\
\hline
\multirow{2}{5em}{BCT} & $\phi_{new}^{bct}/\phi_{old}$  & 41.3-64.4 & 33.3\\
& $\phi_{new}^{bct}/\phi_{new}^{bct}$ & 63.7-79.0 & 51.2\\
\hline
\multirow{2}{5em}{BCT (+32)} & $\phi_{new}^{bct(+32)}/\phi_{old}$ & 37.4-64.4 & 30.0\\
& $\phi_{new}^{bct(+32)}/\phi_{new}^{bct(+32)}$ & 65.7-80.1 & 52.0\\
\hline
\multirow{2}{5em}{contrast} & $\phi_{new}^{contrast}/\phi_{old}$ & 39.0-66.7 & 29.4\\
& $\phi_{new}^{contrast}/\phi_{new}^{contrast}$ & 65.6-81.2 & 47.6\\
\hline
\multirow{2}{5em}{BCT-BX (Ours)} & $\phi_{new}^{bct-bx}/\phi_{old}$ & \textbf{47.8}-\textbf{68.0} & \textbf{33.8}\\
& $\phi_{new}^{bct-bx}/\phi_{new}^{bct-bx}$ & \textbf{66.5}-\textbf{80.9} & \textbf{54.4}\\
\hline
\end{tabular}}
\caption{Backward compatible experiments on imagenet-500 to imagenet-1k with only data change. Both the old model and the new model uses Resnet50-128 architecure.}
\label{table:imagenet data change}
\end{center}
\end{table}
\paragraph{Cifar-50 to Cifar-100} In this experiment, we train $\phi_{old}$ as ResNet50 with outputting feature dimension 128 on Cifar-50 and the new model $\phi_{new}$ on the entire Cifar-100 dataset. For retrieval, we use the Cifar-100 validation set as both the gallery set and the query set.

\paragraph{Imagenet-500 to Imagenet-1k} In this experiment, we train $\phi_{old}$ as ResNet50 with outputting feature dimension 128 on Imagenet-500 and the new model $\phi_{new}$ on the entire Imagenet-1k dataset. For retrieval, we use the Imagenet-1k validation set as both the gallery set and the query set.

\paragraph{Results: } The results of backward compatible experiments with only data change on cifar 100 and imagenet are shown in Table \ref{table:cifar100 data change} and \ref{table:imagenet data change}, where we observe that BCT can indeed achieve backward compatibility on large-scale image classification datasets like imagenet and also achieves reasonable performance of $\phi^{bct}_{new}/\phi^{bct}_{new}$. However, as has also been discussed in the previous literature, $\phi^{bct}_{new}/\phi^{bct}_{new}$ is significantly influenced by the auxiliary influence loss applied while training for BCT. Comparing to the upper bound of training independently, $\phi_{new}'/\phi_{new}'$ of BCT is only 63.7\% and 56.1\% for CMC top 1 on imagenet and cifar100 respectively. Furthermore, the backward compatibility of BCT can be unstable in some of the datasets where we observe that the $\phi^{bct}_{new}/\phi_{old}$ of BCT is only 23.5\% for CMC top 1 on cifar100 while independent $\phi_{old}/\phi_{old}$ is 33.6\% for the same metric. It's unstable performance might be because the influence loss of BCT does not directly encourage the model to be compatible with the old representation, but encouraging it to be compatible with the old classification head, and the inherent conflict of $\phi^{bct}_{new}/\phi_{old}$ and $\phi^{bct}_{new}/\phi^{bct}_{new}$. We also observe a similar pattern for Contrast, indicating that designing a more sophisticated compatibility loss cannot escape from the problems aforementioned. Nonetheless, with the extra dimension introduced by BCT-BX, we observe a significant improvement across the board. In particular, for CMC top 1 on imagenet, BCT-BX achieves 47.8\% for $\phi^{bct-bx}_{new}/\phi_{old}$ and 66.5\% for $\phi_{new}^{bct-bx}/\phi_{new}^{bct-bx}$, 6.5\% and 2.8\% improvement over BCT respectively. It shows that BCT-BX can mitigate the tradeoff between backward compatibility and not hurting new model, by exploiting extra dimensions. We would like to also note that just naively adding new dimension as BCT (+32) does not show a clear improvement over BCT, which additionally exemplifies the importance of strategic exploitation of the extra dimension as we described in Section \ref{sec:merge}.


\subsection{Model Change}
\label{sec:model change}
\paragraph{Cifar-50 to Cifar-100 (ResNet50 to Transformer)} The setting of this experiment is similar to Cifar-50 to Cifar-100 except that the new model is finetuned from a Transformer \cite{DBLP:journals/corr/abs-2010-11929, NIPS2017_3f5ee243} pretrained on entire Imagenet training set. 

\paragraph{Imagenet-500 to Imagenet-1k (ResNet50 to Transformer)} The setting of this experiment is similar to Imagenet-500 to Imagenet-1k except that the new model is finetuned from a Transformer pretrained on entire Imagenet training set.

\paragraph{Results: } The results of backward compatible experiments with both data change and model change from ResNet to transformers on cifar 100 and imagenet are shown in Table \ref{table:cifar100 model change} and \ref{table:imagenet model change}. This is a challenging setting which, to be best of our knowledge, has not been studied in the previous literature. We observe a similar pattern to the data change setting. Again, by designing sophisticated backward compatible loss or naively adding dimensions, as in the case of contrast and BCT (+32), we did not notice a clear improvement. However, by using a strategic exploitation of the extra dimensions, BCT-BX outperforms BCT by 12.5\% and 2.1 \% in terms of CMS top 1 on imagenet over $\phi_{new}^{bct}/\phi_{old}$ and $\phi_{new}^{bct}/\phi_{new}^{bct}$ respectively.


\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ c c c c }
\hline 
\multirow{2}{5em}{Method} & \multirow{2}{3em}{Case} & CMC & \multirow{2}{5em}{mAP@1.0} \\
& & top1-top5 &\\
\hline
\multirow{3}{5em}{Independent} & $\phi_{old}/\phi_{old}$ & 33.6-55.4 & 24.4\\
& $\phi_{new}'/\phi_{old}$ & 0.3-4.7 & 1.7\\
& $\phi_{new}'/\phi_{new}'$ & 89.5-94.3 & 87.5\\
\hline
\multirow{2}{5em}{BCT} & $\phi_{new}^{bct}/\phi_{old}$  & 45.7-83.7  & 32.9\\
& $\phi_{new}^{bct}/\phi_{new}^{bct}$ & 88.7-93.5 & 85.7\\
\hline
\multirow{2}{5em}{BCT (+32)} & $\phi_{new}^{bct(+32)}/\phi_{old}$ & 44.9-\textbf{86.2} & 32.7\\
& $\phi_{new}^{bct(+32)}/\phi_{new}^{bct(+32)}$ & 88.6-93.7 & 84.8\\
\hline
\multirow{2}{5em}{contrast} & $\phi_{new}^{contrast}/\phi_{old}$ & 45.6-81.0 & 32.8\\
& $\phi_{new}^{contrast}/\phi_{new}^{contrast}$ & 88.2-94.0 & 81.9\\
\hline
\multirow{2}{5em}{BCT-BX (Ours)} & $\phi_{new}^{contrast}/\phi_{old}$ & \textbf{51.2}-85.5 & \textbf{34.0}\\
& $\phi_{new}^{contrast}/\phi_{new}^{contrast}$ & \textbf{90.0}-\textbf{94.8} & \textbf{88.4}\\
\hline
\end{tabular}}
\caption{Backward compatible experiments on cifar-50 to cifar-100 with both data change and model change. The old model uses Resnet50-128 architecure, while the new model uses a transformer pretrained on full training set of Imagenet.}
\label{table:cifar100 model change}
\end{center}
\end{table}


\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ c c c c }
\hline 
\multirow{2}{5em}{Method} & \multirow{2}{3em}{Case} & CMC & \multirow{2}{5em}{mAP@1.0} \\
& & top1-top5 &\\
\hline
\multirow{3}{5em}{Independent} & $\phi_{old}/\phi_{old}$ & 43.1-58.3 & 30.9\\
& $\phi_{new}'/\phi_{old}$ & 0.0-0.2 & 0.1\\
& $\phi_{new}'/\phi_{new}'$ & 78.0-87.5 & 72.4\\
\hline
\multirow{2}{5em}{BCT} & $\phi_{new}^{bct}/\phi_{old}$  & 41.1-69.5 & 33.0\\
& $\phi_{new}^{bct}/\phi_{new}^{bct}$ & 74.8-86.7 & 66.5\\
\hline
\multirow{2}{5em}{BCT (+32)} & $\phi_{new}^{bct(+32)}/\phi_{old}$ & 40.5-69.4 & 32.9\\
& $\phi_{new}^{bct(+32)}/\phi_{new}^{bct(+32)}$ & 75.1-87.1 & 66.8\\
\hline
\multirow{2}{5em}{contrast} & $\phi_{new}^{contrast}/\phi_{old}$ & 43.5-71.3 & 34.0\\
& $\phi_{new}^{contrast}/\phi_{new}^{contrast}$ & 72.5-86.3 & 58.5\\
\hline
% \multirow{2}{5em}{BCT-BX  (+32)} & $\phi_{new}/\phi_{old}$ & 39.4-63.8 & 30.3\\
% & $\phi_{new}/\phi_{new}$ & 71.9-84.6 & 60.5\\
% \hline
\multirow{2}{5em}{BCT-BX (+32)} & $\phi_{new}^{bct-bx}/\phi_{old}$ & \textbf{53.6}-\textbf{74.5} & \textbf{37.5}\\
& $\phi_{new}^{bct-bx}/\phi_{new}^{bct-bx}$ & \textbf{76.9}-\textbf{88.2} & \textbf{70.4}\\
\hline
\end{tabular}}
\caption{Backward compatible experiments on imagenet-500 to imagenet-1k with both data change and model change. The old model uses Resnet50-128 architecure, while the new model uses a transformer pretrained on full training set of Imagenet21K.}
\label{table:imagenet model change}
\end{center}
\end{table}

\subsection{Modality Change}
\label{sec:modality change}
\paragraph{Setting: } In addition to data and model change, we propose an even more challenging situation of modality change, which generalizes the idea of backward compatibility to new potential applications. We consider the application of modality fusion, where a single gallery of image represetations can support both image-to-image retrieval and image-to-text retrieval. In a standard setting, this needs to be done with two separate models: one trained for good image representations (with classification loss on a large-scale image datasets for example) and the other one trained to align the representations of images and text in the same representation space. The first model can only be used for image-to-image retrieval, and the second one, although supports good image-to-text matching, is much worse than the first one in terms of image to image retrieval \yifei{will add some results on this}. This can be considered as a generalization of backward compatible training, where we aim at training a new representation model that supports both the query of images and text, i.e. that is compatible with both the image-to-image retrieval model and text-to-image retrieval. In this setting, we take the text-to-image representation model as the old model and would like to train a new model that attains the ability of image-to-image retrieval while being backward compatible the the text-to-image representation model. This is extremely challenging because the old model is a text model while the new model is an image model.

To simulate experiments in this setting, we use a pretrained GPT2 \cite{Radford2019LanguageMA} image captioning model to automatically generate captions for all images in imagenet with "vit-gpt2-image-captioning" from \cite{DBLP:journals/corr/abs-1910-03771}. We use the text model of CLIP \cite{DBLP:journals/corr/abs-2103-00020} as our old model and a pretrained Visual Transformer \cite{DBLP:journals/corr/abs-2010-11929} finetuned on imagenet-1k classification as our new model. We measure the performances of different baselines and our method by $\phi_{clip-text}/\phi_{new}$ and $\phi_{new}/\phi_{new}$, which is the performances of text-to-image and image-to-image retrievals. As a benchmark comparison, we use $\phi_{clip-text}/\phi_{clip-image}$ to denote the text-to-image retrieval performance with CLIP text model and CLIP image model.

\paragraph{Results: } First, we notice that the performance of $\phi_{clip-text}/\phi_{clip-image}$, where we measure to text-to-image retrieval performance with CLIP text model and CLIP image model, is relatively low compared to other models. This is mainly because we use automatic image captioning instead of manually annotated ones to caption the text descriptions associated with each image, so many of them are not accurate. Second, because of the challenge of modality change and noise in the training data, BCT and contrast fail to achieve backward compatibility (CMC top 1 of $\phi_{clip-text}/\phi_{new}^{bct}$ is 9.1\% compared to 11.7\% of $\phi_{clip-text}/\phi_{clip-image}$) and the performance of $\phi_{new}^{bct}/\phi_{new}^{bct}$ is also significantly hurt by 4.4\% (CMC top 1 of 73.7\% compared to 78.0\%). Finally, we observe that BCT-BX is particularly robust in this setting with rigorous backward compatibility (CMC top 1 11.4\% compared to 11.7\%) and marginal loss in $\phi_{new}^{bct-bx}/\phi_{new}^{bct}-bx$ (CMC top 1 77.6\% compared to 78.0\%). We also want to note that different from the experiments of data change and model change, we set the dimension of $\phi_{new}^{bct}$ and $\phi_{clip-text}$ to be 512, the same as the dimension of CLIP while still managed to keep the dimension expansion of $\phi_{new}^{bct-bx}$ as only 32. It shows that our BCT-BX is extremely dimension efficient in the sense that we only need to expand the dimension by 6.25\%.

% \begin{table}
% \label{table:cifar100 modality change}
% \begin{center}
% \begin{tabular}{ c c c c }
% \hline 
% \multirow{2}{5em}{Method} & \multirow{2}{3em}{Case} & CMC & \multirow{2}{5em}{mAP@1.0} \\
% & & top1-top5 &\\
% \hline
% \multirow{3}{5em}{Independent} & $\phi_{old}/\phi_{old}$ & 30.1-50.1 & 19.3\\
% & $\phi_{new}/\phi_{old}$ &  &\\
% & $\phi_{new}/\phi_{new}$ & 89.5-94.3 & 87.5\\
% \hline
% \multirow{2}{5em}{BCT} & $\phi_{new}/\phi_{old}$  &  & \\
% & $\phi_{new}/\phi_{new}$ &  & \\
% \hline
% \multirow{2}{5em}{BCT (+32)} & $\phi_{new}/\phi_{old}$ &  & \\
% & $\phi_{new}/\phi_{new}$ &  & \\
% \hline
% \multirow{2}{5em}{contrast} & $\phi_{new}/\phi_{old}$ & ( & )\\
% & $\phi_{new}/\phi_{new}$ &(& )\\
% \hline
% \multirow{2}{5em}{BCT-BX (Ours)} & $\phi_{new}/\phi_{old}$ & 42.6-78.0 & 32.1\\
% & $\phi_{new}/\phi_{new}$ & 90.2-94.7 & 88.8\\
% \hline
% \end{tabular}
% \caption{Backward compatible experiments on cifar-50 to cifar-100 with modality change. The old model uses a pretrained CLIP text encoder with automatically generated text, while the new model uses a transformer pretrained on full training set of Imagenet21K.}
% \end{center}
% \end{table}

\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ c c c c }
\hline 
\multirow{2}{5em}{Method} & \multirow{2}{3em}{Case} & CMC & \multirow{2}{5em}{mAP@1.0} \\
& & top1-top5 &\\
\hline
\multirow{3}{5em}{Independent} & $\phi_{clip-text}/\phi_{clip-image}$ & 11.7-25.0 & 7.0\\
& $\phi_{clip-text}/\phi_{new}'$ & 0.1-0.4 & 0.3\\
& $\phi_{new}'/\phi_{new}'$ & 78.0-87.5 & 72.4\\
\hline
\multirow{2}{5em}{BCT} & $\phi_{clip-text}/\phi_{new}^{bct}$  & 9.1-21.4 & 12.1\\
& $\phi_{new}^{bct}/\phi_{new}^{bct}$ & 73.7-85.9 & 65.9\\
\hline
\multirow{2}{5em}{BCT (+32)} & $\phi_{clip-text}/\phi_{new}^{bct(+32)}$ & 9.2-21.8 & 12.1\\
& $\phi_{new}^{bct(+32)}/\phi_{new}^{bct(+32)}$ & 73.8-85.5 & 65.5\\
\hline
\multirow{2}{5em}{contrast} & $\phi_{clip-text}/\phi_{new}^{contrast}$ & \textbf{13.0}-\textbf{30.0} & 8.8\\
& $\phi_{new}^{contrast}/\phi_{new}^{contrast}$ & 48.0-68.2 & 23.1\\
\hline
\multirow{2}{5em}{BCT-BX (Ours)} & $\phi_{clip-text}/\phi_{new}^{bct-bx}$ & 11.4-25.6 & \textbf{13.6}\\
& $\phi_{new}^{bct-bx}/\phi_{new}^{bct-bx}$ & \textbf{77.6}-\textbf{87.4} & \textbf{71.5}\\
\hline
\end{tabular}}
\caption{Backward compatible experiments on Imagenet-500 to Imagenet-1k with modality change. The old model uses a pretrained CLIP text encoder with automatically generated text, while the new model uses a transformer pretrained on full training set of Imagenet21K.}
\label{table:imagenet modality change}
\end{center}
\end{table}


\subsection{Series of Model Updates}
To simulate the real-world scenario where often new models might come in series, we also test our methodology in a series of model updates. In particular, we simulate the evolution of neural network architectures in the past decade (2010-2022). Our first model architecture is AlexNet \cite{NIPS2012_c399862d}, followed by VGGNet13 \cite{simonyan2014very}, ResNet50 \cite{DBLP:journals/corr/HeZRS15}, and finally ViT \cite{DBLP:journals/corr/abs-2010-11929}. All models are trained on Imagenet-1k training and results are tested on Imagenet-1k validation set. Our BCT-BX adds 32 extra dimensions for each update, all other models use an embedding size of 128.

\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ c c c c }
\hline 
\multirow{2}{5em}{Method} & \multirow{2}{3em}{Case} & CMC & \multirow{2}{5em}{mAP@1.0} \\
& & top1-top5 &\\
\hline
\multirow{4}{5em}{Independent} & $\phi_{alex}/\phi_{alex}$ & 46.6-66.3 & 29.1\\
& $\phi_{vgg}/\phi_{vgg}$ & 63.2-79.0 & 49.6\\
& $\phi_{res}/\phi_{res}$ & 67.9-81.4 & 52.3\\
& $\phi_{vit}/\phi_{vit}$ & 78.0-87.5 & 72.4\\
\hline
\multirow{9}{5em}{BCT} & $\phi_{vgg}^{bct}/\phi_{alex}$  & 54.4-74.1 & 36.2\\
& $\phi_{vgg}^{bct}/\phi_{vgg}^{bct}$ & 58.4-75.4 & 47.0\\
& $\phi_{res}^{bct}/\phi_{alex}^{bct}$ & 46.0-71.9 & 30.6\\
& $\phi_{res}^{bct}/\phi_{vgg}^{bct}$ & 48.9-75.2 & 44.4\\
& $\phi_{res}^{bct}/\phi_{res}^{bct}$ & 64.3-79.1 & 52.7\\
& $\phi_{vit}^{bct}/\phi_{alex}^{bct}$ & 54.9-82.0 & 36.3\\
& $\phi_{vit}^{bct}/\phi_{vgg}^{bct}$ & 57.5-84.1 & 50.5\\
& $\phi_{vit}^{bct}/\phi_{res}^{bct}$ & 70.3-85.1 & 57.0\\
& $\phi_{vit}^{bct}/\phi_{vit}^{bct}$ & 73.9-86.0 & 65.8\\
\hline
\multirow{9}{5em}{BCT-BX (ours)} & $\phi_{vgg}^{bct-bx}/\phi_{alex}$  & \textbf{56.5}-\textbf{75.6} & \textbf{37.1}\\
& $\phi_{vgg}^{bct-bx}/\phi_{vgg }^{bct-bx}$ & \textbf{61.0}-\textbf{77.2} & \textbf{48.5}\\
& $\phi_{res}^{bct-bx}/\phi_{alex}^{bct-bx}$ & \textbf{56.7}-\textbf{78.5} & \textbf{37.2}\\
& $\phi_{res}^{bct-bx}/\phi_{vgg}^{bct-bx}$ & \textbf{61.5}-\textbf{80.8} & \textbf{50.6}\\
& $\phi_{res}^{bct-bx}/\phi_{res}^{bct-bx}$ & \textbf{66.6}-\textbf{80.8} & \textbf{56.8}\\
& $\phi_{vit}^{bct-bx}/\phi_{alex}^{bct-bx}$ & \textbf{57.9}-\textbf{83.5} & \textbf{37.6}\\
& $\phi_{vit}^{bct-bx}/\phi_{vgg}^{bct-bx}$ & \textbf{62.5}-\textbf{86.5} & \textbf{52.7}\\
& $\phi_{vit}^{bct-bx}/\phi_{res}^{bct-bx}$ & \textbf{72.0}-\textbf{87.0} & \textbf{60.6}\\
& $\phi_{vit}^{bct-bx}/\phi_{vit}^{bct-bx}$ & \textbf{75.6}-\textbf{87.4} & \textbf{68.0}\\
\hline
\end{tabular}}
\caption{Backward compatible experiments on a series of model updates on Imagenet-1k. Our BCT-BX adds 32 extra dimensions for each update, all other models use an embedding size of 128.}
\label{table: a series of updates}
\end{center}
\end{table}

\paragraph{Results: }The results of sequential updates of the model architecture are shown in Table \ref{table: a series of updates}. Note that because BCT (+32) and contrast did not show clear advantage over BCT in previous experiments, we only compare our method with BCT here. We first note the failure of BCT in this challenging setting. In the first update from AlexNet to VGGNet13, although backward compatiblility is achieved (for Top1, $\phi_{vgg}^{bct}/\phi_{alex}$ is 54.1\% while independent $\phi_{alex}/\phi_{alex}$ is 46.6\%), the performance of $\phi_{vgg}^{bct}/\phi_{vgg}^{bct}$ is significantly hurt (for Top1, $\phi_{vgg}^{bct}/\phi_{vgg}^{bct}$ is 58.4\% while independent $\phi_{vgg}/\phi_{vgg}$ is 63.2\%). Furthermore, after another round of update in model architecture from VGGNet13 to ResNet50, the model does not maintain a decent backward compatibility with its former versions $\phi_{alex}$ and $\phi^{bct}_{vgg}$ with a loss of 0.6\% in $\phi_{res}^{bct}/\phi_{alex}^{bct}$ and 4.3\% in $\phi_{res}^{bct}/\phi_{vgg}^{bct}$ compared to independent $\phi_{alex}/\phi_{alex}$ and $\phi_{vgg}/\phi_{vgg}$ in Top1. Although its backward compatibility is improved after updating to $\phi^{bct}_{vit}$ possibly because of the power of pretraining for ViT, it still hurts the performance of the new model significantly (for Top1, $\phi^{bct}_{vit}/\phi^{bct}_{vit}$ is only 73.9\% compared to independent $\phi_{vit}/\phi_{vit}$ with 78.0\%). On the contrast, we observe that by a strategic use of extra dimensions, our BCT-BX maintains backward compatibility at each stage of the sequential updates and closes the gap between the performance of the independent new models and the models trained with BCT. Thus we see that our BCT-BX shows a clear advantage on all rows across the board with gains up to 17.7\%.

\section{Ablations on the Number of Extra Dimensions}
\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ c c c c }
\hline 
\multirow{2}{5em}{Method} & \multirow{2}{3em}{Case} & CMC & \multirow{2}{5em}{mAP@1.0} \\
& & top1-top5 &\\
\hline
\multirow{3}{5em}{Independent} & $\phi_{old}/\phi_{old}$ & 43.1-58.3 & 30.9\\
& $\phi_{new}'/\phi_{old}$ & 0.0-0.2 & 0.1\\
& $\phi_{new}'/\phi_{new}'$ & 78.0-87.5 & 72.4\\
\hline
\multirow{2}{5em}{BCT} & $\phi_{new}^{bct}/\phi_{old}$  & 41.1-69.5 & 33.0\\
& $\phi_{new}^{bct}/\phi_{new}^{bct}$ & 74.8-86.7 & 66.5\\
\hline
 \multirow{2}{5em}{BCT-BX (+8)} & $\phi_{new}^{+8}/\phi_{old}$ & 50.7-75.9 & 37.1\\
& $\phi_{new}^{+8}/\phi_{new}^{+8}$ & 74.8-87.0 & 66.0\\
\hline
\multirow{2}{5em}{BCT-BX (+16)} & $\phi_{new}^{+16}/\phi_{old}$ & 51.6-\textbf{76.1} & 37.6\\
& $\phi_{new}^{+16}/\phi_{new}^{+16}$ & 76.4-88.1 & 69.0\\
\hline
\multirow{2}{5em}{BCT-BX (+32)} & $\phi_{new}^{+32}/\phi_{old}$ & \textbf{53.6}-74.5 & 37.5\\
& $\phi_{new}^{+32}/\phi_{new}^{+32}$ & 76.9-88.2 & 70.4\\
\hline
\multirow{2}{5em}{BCT-BX (+128)} & $\phi_{new}^{+128}/\phi_{old}$ & 53.4-75.0 & \textbf{37.9}\\
& $\phi_{new}^{+128}/\phi_{new}^{+128}$ & \textbf{77.8}-\textbf{88.5} & \textbf{71.1}\\
\hline
\end{tabular}}
\caption{Dimension ablation experiments on imagenet-500 to imagenet-1k with both data change and model change. The old model uses Resnet50-128 architecure, while the new model uses a transformer pretrained on full training set of Imagenet21K. Our BCT-BX adds 32 extra dimensions for each update, all other models use an embedding size of 128.}
\label{table:dimension ablations}
\end{center}
\end{table}

To answer the last question on how much dimension is needed for BCT-BX, we carry out ablation experiments in the setting of ResNet50 to ViT (with both data change and model change) on Imagenet-1k. All settings are the same as in Section \ref{sec:model change} except we vary the number of extra dimensions in our BCT-BX. Results of the ablations are shown in Table \ref{table:dimension ablations}, where we compare BCT (no extra dimension) with BCT-BX extra 8, 16, 32, 128 dimensions. We observe that BCT-BX already shows a clear advantage over BCT with as few as 8 extra dimensions, showing the effectiveness of our proposed Basis Transformation Block. As extra dimensions grow from 8 to 32, though less significant, we observe an overall trend of gradual improvement both in terms of both $\phi_{new}^{+n}/\phi_{new}^{+n}$ and $\phi_{new}^{+n}/\phi_{old}$. As a result, the CMC top 1 of BCT-BX (+32) is 2.7\% and 2.1\% higher than BCT-BX (+32) in terms of $\phi_{new}^{+n}/\phi_{new}^{+n}$ and $\phi_{new}^{+n}/\phi_{old}$ respectively. Finally, we notice that the improvement from BCT-BX (+32) to BCT-BX (+128) is somewhat marginal by -0.2\% and 0.9\% in terms of $\phi_{new}^{+n}/\phi_{new}^{+n}$ and $\phi_{new}^{+n}/\phi_{old}$ respectively. Note that BCT-BX (+128) is similar to the upperbound solution in that it shares 0 dimension of $\phi_{old}'$ and $\phi_{new}'$ and just concatenate them together. This result shows that some of the information of $\phi_{new}'$ and $\phi_{old}'$ can be shared so that we do not have to concatenate them to retain the full information of both $\phi_{new}'$ and $\phi_{old}'$.

==> CVPR_submission/intro_back.tex <==
\section{Introduction}
\label{sec:intro}
Modern visual representation retrieval systems involves retrieving similar images from a giant pool of stored data (referred as gallery) with an given image (referred as query). This is often done by training a representation model to encode all the images in the gallery and save them. During inquery, we first encode the query and retrieve the images with the most similar saved representations. However, as new data comes in and better model architectures start to be available, often we will need to update the model for better performances. The issue is that if the new model is trained independently from the old model, the representations generated by the new model will not be compatible with those generated the old model, which necessitates re-calculating the representations of the gallery set, a process known as "back-filling"  \cite{9156906}. This process can be very costly given the giant scale of the gallery set, and even impossible if in reality the original image is deleted due to privacy concern.

Shen \etal \cite{9156906} therefore proposes a framework to train the new model while being compatible with the old model, known as Backward Compatible Training (BCT), with the hope of removing the need of back-filling. They propose to add an "influence loss" to the training objective of the new model to heuristically induce a backward-compatible representation (following a standard notation, we use $\phi^1/\phi^2$ to represent the retrieval performance of using $\phi^1$ as query representations while using $\phi^2$ as gallery representations. and we denote the old representation model as $\phi_{old}$ and the new representation model as $\phi_{new}$) . However, as pointed out by \cite{ramanujan2022forward}, adding this influence loss can significantly hurt the performance of the new model, that is $\phi_{new}/\phi_{new}$. To mitigate this issue, following-up works have tried to design a more sophisticated influence loss that empirically induces a backward-compatible representation while minimally hurting the performance of the new model \cite{DBLP:journals/corr/abs-2201-09724, DBLP:journals/corr/abs-2108-01958, https://doi.org/10.48550/arxiv.2203.01583}. However, limited progress has been achieved in the first direction. Indeed, as shall be detailed in \ref{sec:tradeoff}, it can be impossible to find a new representation model that is at the same time backward compatible and achieves the fullest potential of the new model. We also notice that sometimes thanks to the new model architecture or new data, using the new representation to retrieve old representations in the gallery can be even better than using the old representation to retrieve its own representations in the gallery, as reported by Shen \etal \cite{9156906}. Therefore, forcing both the loss to induce backward compatibility (that is, to maximize $\phi_{new}/\phi_{old}$) and the loss to train the new model (that is, to maximize $\phi_{new}/\phi_{new}$) will not only restrict the potential of the new model on its own but also restrict the new model's capability to retrieve old representations. In other words, it is hard to train a single representation that maximizes both $\phi_{new}/\phi_{new}$ and $\phi_{new}/\phi_{old}$. Therefore, researchers propose to avoid the inherent tradeoff between backward compatibility and new model capacity by introducing a light-weight transformation of the old representation into the new representation \cite{DBLP:journals/corr/abs-2008-04821, ramanujan2022forward, https://doi.org/10.48550/arxiv.2204.13919}. Despite their effort to make the transformation light-weight, it still requires applying a neural network to update billions of images in the gallery, which can still be costly. Furthermore, the old model architecture might not be able to capture and save some of the information that will be used by the new model architecture, meaning that an ideal transformation from the old model to the new model might not always be possible. \yifei{I'll try to run some experiments to show this.}

% However, neither of the two categories manage to provide a rigorous guarantee of backward compatibility, as discussed by Shen \etal \cite{9156906}, backward compatible training with heuristic influence loss might fail in case of large distribution shift or large changes in the model architecture. 

% Furthermore, both of the two categories restrict the potential of the new model. On one hand, adding a new influence loss prevents the new model from learning a representation as well as it should \cite{ramanujan2022forward}. On the other hand, transforming from an old representation to a new representation is subject to the encoding ability of the old model \cite{DBLP:journals/corr/abs-2008-04821} and side-information model \cite{ramanujan2022forward}. This is undesirable, since oftentimes we cannot estimate what new models we will be using in advance while deploying the old model.

% In this paper, we propose Spectral Backward Compatible Training (Spectral BCT) to aim at \emph{rigorously providing backward compatible representations without restricting the performance of the new model}, and requiring no transformations from the old representation to new ones. The intuition behind Spectral BCT is to grow the new representation in the near orthogonal direction of the space made of the old representations. Therefore, if we compare the new representation with the old representation, the orthogonal components cancel so that it behaves exactly like the old representation, and if we properly set the ratio of the new representation on the orthogonal basis to the old representation, we can achieve the fullest potential of the new model. 

Despite the inherent conflict between backward compatibility and new model capacity, we notice that this conflict can be reconciled if we can expand the representation space, so that it is large and powerful enough to contain both the best backward compatible model and the best independently trained new model. As a naive solution, if we train a model $\phi_{new}'$ independently without considering backward compatibility (that is only to maximize $\phi_{new}'/\phi_{new}'$) and train a model $\phi_{old}'$ only considering backward compatibility (that is only to maximize $\phi_{old}'/\phi_{old}$). In this way, since both of the two models are trained independently, we avoid the issue of tradeoffs between $\phi_{new}/\phi_{new}$ and $\phi_{new}/\phi_{old}$ if we were to tain a single model $\phi_{new}$. Therefore, $\phi_{new}'$ realizes the best possible $\phi_{new}'/\phi_{new}'$ and $\phi_{old}'$ realizes the best possible $\phi_{old}'/\phi_{old}$. To assemble $\phi_{new}'$ and $\phi_{old}'$, we simply concatenate them and define:
\begin{align*}
    \phi_{new} = \begin{bmatrix}
\phi_{old}'  \\
c \times \phi_{new}'  
\end{bmatrix},
\end{align*}
where $c$ is an arbitrary constant. While retrieval, we consider the distance metric $d$ as negative dot product and truncate a vector if it has a larger dimension than the other vector while doing the dot product. In this way, for any $x_1, x_2$, if we consider $d(\phi_{new}(x_1),\phi_{old}(x_2))$, all the $\phi_{new}'(x_1)$ are on the extra orthogonal dimension and therefore truncated so it is equivalent to $d(\phi_{old}'(x_1),\phi_{old}(x_2))$, so it achieves the best possible $\phi_{new}/\phi_{old}$. If we consider $d(\phi_{new}(x_1), \phi_{new}(x_2))$, it is equal to $d(\phi_{old}'(x_1), \phi_{old}'(x_2))+ c^2d(\phi_{new}'(x_1), \phi_{new}'(x_2))$ and if we set $c$ large enough, $d(\phi_{new}'(x_1), \phi_{new}'(x_2))$ will be the dominant term so it also achieves the best possible $\phi_{new}/\phi_{old}$.

% and apply a change to basis to transform the representations $\phi'$ to be orthogonal to the old representations $\phi_{old}$ (adding new dimension if necessary) and add that orthogonal part to the old model to be the new model $\phi_{new} = c*\phi' + \phi_{old}$ (where c is a constant that can be set to adjust the ratio of $\phi'$ and $\phi_{old}$), so that we also preserves the best possible performance of the new model (i.e. when trained independently) while keeping backward compatible. 

\begin{figure}[!ht]
  \centering
   \includegraphics[width=0.8\linewidth]{BCT_failure.pdf}

   \caption{An example of where BCT with influence loss fail to provide a backward compatible guarantee or leave room for new model update while our method is not affected. Red points and blue points correspond to old representations of different classes.}
   \label{intuition}
\end{figure}

In Figure \ref{intuition}, we show an example to illustrate intuition of adding new dimensions to get over the inherent tradeoff between $\phi_{new}/\phi_{old}$ and $\phi_{new}/\phi_{new}$. Applying an influence loss encourages the new model to learn a representation close to the center of a old representations of a specific class, while the intuition of the naive solution is to encourage the model to mimic the old model in its main dimensions while growing on the orthogonal directions. In the scenario below where red and blue points correspond to old embeddings of different classes, yellow arrows correspond to the direction where the new representations tend to move with the influence loss while green arrows denote the direction where the new representations tend to move with our naive solution. As shown in the figure, the influence loss not only limits the potential of the new model because of the constraints of the old representations but also incurs a mistake of retrieval because the blue points in the middle will get closer to some red points. On the other hand, if we move perpendicular to the old representations, as is the case of our naive solution, we're free to develop our new model while being rigorously compatible with the old representations. 

Although this naive solution achieves the desired property of the best possible new model with rigorous backward compatibility, it is faced with two critical drawbacks. First of all, the computation of $\phi_{new}$ requires two independent models $\phi_{old}'$ and $\phi_{new}'$, which nearly doubles the computations required to calculate every new representation. Secondly, we also observe a significant dimension expansion because we might have to double the dimension if the dimension of $\phi_{old}'$ is the same as that of $\phi_{new}'$. Those two drawbacks significantly increase the computational and storage cost of the naive solution, preventing it from actually being useful in practice. To address those two drawbacks, we propose Spectral Backward Compatible Training (Spectral BCT), which not only achieves nearly the best possible new model with rigorous backward compatibility, but also avoids the issue of requiring two models and doubling the representation space. 

Specifically, to address the first concern, we train a new backbone and distill $\phi_{new}'$ and $\phi_{old}'$ into different layers, so that by only one forward pass, we can get both $\phi_{new}'$ and $\phi_{old}'$. To address the second concern, we notice that despite the possible difference in the training and model architecture between $\phi_{new}'$ and $\phi_{old}'$ (for example, transformers and ResNet), they should have still encoded a considerable amount of shared information (like colors, shapes, and so on for images). It would be a waste of dimension if we duplicate that information. Therefore, we propose to use a series of transformations to automatically pick out the shared information of $\phi_{old}'$ and $\phi_{new}'$, and only put the extra information introduced by $\phi_{new}'$ on the extra orthogonal basis, so that we can significantly reduce the expansion of dimension in practice (up to 75\%-95\%). In particular, we choose a series of learnable change of basis as the transformation due to the observation that change of basis transformation can preserve all the information in the original embeddings (and dot product between two representations is invariant to this type of transformation).

% However, since $\phi_{new}$ is an ensemble of two models, to save the computational cost, we need to distill the knowledge of the two models into one. To this end, we propose a novel knowledge distillation framework for multiple representation learning models, where we distill different models into different layers of the distilled model and ensemble representations from different layers during inference time. In this way, we manage to derive $\phi_{new}$ with only one pass of the representation model. In many practical situations, we may not have the luxury of growing entirely on the orthogonal direction of the old representation space due to its large increase in the representation space. To this end, we propose a novel learnable change of basis to automatically identify and make use of the shared information in the old and new representation model, and only growing the extra information on the orthogonal direction, with a similar rigorous theoretical guarantee.

In short, our contributions are three-fold:
\begin{enumerate}
    \item We propose spectral BCT for backward compatible representation learning, and show that it not only guarantees backward compatibility but also exploits the new model in its fullest potential. Moreover, the framework of BCT is general enough to work in a broader setting than the previous literature, including a series of model updates and fusing models with different modalities.
    
    \item To overcome the problem of increasing computational cost and storage of the naive solution, we introduce a novel method of a trainable change of basis with extra information to achieve both backward compatibility and not hurting new model by distilling different models into different layers of the distilled model and assembling them by trainable changes of basis.
    \item We support our framework with strong empirical evidence of guaranteeing backward compatibility while minimally hurting the new model, stably outperforming other state-of-the-art methods with a large margin.
\end{enumerate}

==> CVPR_submission/introduction.tex <==
\section{Introduction}
\label{sec:intro}
Modern visual representation retrieval systems involves retrieving similar images from a giant pool of stored data (referred as gallery) with an given image (referred as query). This is often done by training a representation model to encode all the images in the gallery and save them. During inquiry, we first encode the query and retrieve the images with the most similar saved representations. However, as new data comes in and better model architectures start to be available, often we will need to update the model for better performances. The issue is that if the new model is trained independently from the old model, the representations generated by the new model will not be compatible with those generated the old model, which necessitates re-calculating the representations of the gallery set, a process known as "back-filling"  \cite{9156906}. This process can be very costly given the giant scale of the gallery set, and even impossible if in reality the original image is deleted due to privacy concern.

Shen \etal \cite{9156906} therefore proposes a framework to train the new model while being compatible with the old model, known as Backward Compatible Training (BCT), with the hope of removing the need of back-filling. They propose to add an "influence loss" to the training objective of the new model to heuristically induce a backward-compatible representation (following a standard notation, we use $\phi^1/\phi^2$ to represent the retrieval performance of using $\phi^1$ as query representations while using $\phi^2$ as gallery representations. and we denote the old representation model as $\phi_{old}$ and the new representation model as $\phi_{new}$) . However, as pointed out by \cite{ramanujan2022forward}, adding this influence loss can significantly hurt the performance of the new model, that is $\phi_{new}/\phi_{new}$. To mitigate this issue, following-up works have tried to design a more sophisticated influence loss that empirically induces a backward-compatible representation while minimally hurting the performance of the new model \cite{DBLP:journals/corr/abs-2201-09724, DBLP:journals/corr/abs-2108-01958, https://doi.org/10.48550/arxiv.2203.01583}. However, limited progress has been achieved in the first direction. Indeed, as shall be detailed in \ref{sec:tradeoff}, it can be impossible to find a new representation model that is at the same time backward compatible and achieves the fullest potential of the new model. We also notice that sometimes thanks to the new model architecture or new data, using the new representation to retrieve old representations in the gallery can be even better than using the old representation to retrieve its own representations in the gallery, as reported by Shen \etal \cite{9156906}. Therefore, forcing both the loss to induce backward compatibility (that is, to maximize $\phi_{new}/\phi_{old}$) and the loss to train the new model (that is, to maximize $\phi_{new}/\phi_{new}$) will not only restrict the potential of the new model on its own but also restrict the new model's capability to retrieve old representations. In other words, it is hard to train a single representation that maximizes both $\phi_{new}/\phi_{new}$ and $\phi_{new}/\phi_{old}$. Therefore, researchers propose to avoid the inherent tradeoff between backward compatibility and new model capacity by introducing a light-weight transformation of the old representation into the new representation \cite{DBLP:journals/corr/abs-2008-04821, ramanujan2022forward, https://doi.org/10.48550/arxiv.2204.13919}. Despite their effort to make the transformation light-weight, it still requires applying a neural network to update billions of images in the gallery, which can be costly. 

Despite the inherent conflict between backward compatibility and new model capacity, we notice that this conflict can be reconciled if we can expand the representation space, so that it is large and powerful enough to contain both the best backward compatible model and the best independently trained new model. As an upper bound solution, if we train a model $\phi_{new}'$ independently without considering backward compatibility (that is only to maximize $\phi_{new}'/\phi_{new}'$) and train a model $\phi_{old}'$ only considering backward compatibility (that is only to maximize $\phi_{old}'/\phi_{old}$). In this way, since both of the two models are trained independently, we avoid the issue of tradeoffs between $\phi_{new}/\phi_{new}$ and $\phi_{new}/\phi_{old}$ if we were to tain a single model $\phi_{new}$. Therefore, $\phi_{new}'$ realizes the best possible $\phi_{new}'/\phi_{new}'$ and $\phi_{old}'$ realizes the best possible $\phi_{old}'/\phi_{old}$. To assemble $\phi_{new}'$ and $\phi_{old}'$, we simply concatenate them and define:
\begin{align*}
    \phi_{new} = \begin{bmatrix}
\phi_{old}'  \\
c \times \phi_{new}'  
\end{bmatrix},
\end{align*}
where $c$ is an arbitrary constant. While retrieval, we consider the distance metric $d$ as negative dot product and truncate a vector if it has a larger dimension than the other vector while doing the dot product. In this way, for any $x_1, x_2$, if we consider $d(\phi_{new}(x_1),\phi_{old}(x_2))$, all the $\phi_{new}'(x_1)$ are on the extra orthogonal dimension and therefore truncated so it is equivalent to $d(\phi_{old}'(x_1),\phi_{old}(x_2))$, so it achieves the best possible $\phi_{new}/\phi_{old}$. If we consider $d(\phi_{new}(x_1), \phi_{new}(x_2))$, it is equal to $d(\phi_{old}'(x_1), \phi_{old}'(x_2))+ c^2d(\phi_{new}'(x_1), \phi_{new}'(x_2))$ and if we set $c$ large enough, $d(\phi_{new}'(x_1), \phi_{new}'(x_2))$ will be the dominant term so it also achieves the best possible $\phi_{new}/\phi_{old}$.

Although this upperbound solution achieves the desired property of the best possible new model with rigorous backward compatibility, it is faced with two critical drawbacks. First of all, the computation of $\phi_{new}$ requires two independent models $\phi_{old}'$ and $\phi_{new}'$, which nearly doubles the computations required to calculate every new representation. Secondly, we also observe a significant dimension expansion because we might have to double the dimension if the dimension of $\phi_{old}'$ is the same as that of $\phi_{new}'$. Those two drawbacks significantly increase the computational and storage cost of the naive solution, preventing it from actually being useful in practice. However, this upper bound solution inspires us to consider adding new dimensions to the representation space to get over the tradeoff between $\phi_{new}/\phi_{old}$ and $\phi_{new}/\phi_{new}$.

We first tried naively adding dimensions only to the new representation without changing anything else in the previous influence loss method proposed by Shen \etal \cite{9156906}, where we set the dimension of $\phi_{old}$ to be 128 while the dimension of $\phi_{new}$ to be 160, but were surprised to find that this did not lead to a clear advantage as shown in Section \ref{sec:experiments}. We observe that in $\phi_{new}$, the first 128 dimensions where the influence loss is applied have more information (in terms of the average norm) than the extra 32 dimensions, possibly indicating the influence loss prevents the naive solution to effectively make use of the extra dimensions. 

In an ideal scenario, we would like our model $\phi_{new}$ to contain both the information of $\phi_{new}'$ and $\phi_{old'}$ (as our upperbound solution does), putting $\phi_{old'}$ on the first 128 dimensions and the information of $\phi_{new}'$ that is not compatible with $\phi_{old}$ on the extra 32 dimensions. Towards this end, we propose a novel framework of Basis Transformation Block (BX) that exploits a series of learnable change of basis to automatically learn to find the information of $\phi_{new}'$ that is not compatible with $\phi_{old}$ on the extra 32 dimensions, while maintaining the information of $\phi_{new}'$ and $\phi_{old}'$. This is achieved by the favorable property of learnable change of basis that it will not change the information stored in a representation (formally stated in Lemma \ref{lemma:change of basis}). We empirically verify that our Basis Transformation Block can effectively exploit the extra dimensions given to $\phi_{new}$ and establish a significant advantage over BCT and other current state-of-the-art backward compatible training methods. Our method is shown to be effective not only in some standard backward compatible training settings like data change, but also in many more challenging and practical settings like significant model change (for example, ResNet to Transformers), modality change and a series of updates in model architecture in the history of the past decade. 

In short, our contributions are three-fold:
\begin{enumerate}
    \item We provide the research insight of the inherent tradeoff between $\phi_{new}/\phi_{old}$ and $\phi_{new}/\phi_{new}$ and that it can be reconciled with extra dimensions for $\phi_{new}$.
    
    \item We propose Backward Compatible Training with Change of Basis Block (BCT-BX), that exploits a series of learnable change of basis to effectively exploit the extra dimensions, and verify its empirical advantage over other state-of-the-art methods in a wide range of backward compatible training settings.
    
    \item We extend the success our BCT-BX to more challenging scenarios that have not been considered by existing works to the best of our knowledge such as significant change in model architecture, modality change, and even a series of updates in the model architecture mimicing the histroy of the past decade, which has not been studies in existing works to the best of our knowledge. We show that those new settings not only are more practical to the real-world use but also inspire novel applications of BCT in practice like enabling information retrieval of the same representation with queries from different modalities.
    % \item We propose spectral BCT for backward compatible representation learning, and show that it not only guarantees backward compatibility but also exploits the new model in its fullest potential. Moreover, the framework of BCT is general enough to work in a broader setting than the previous literature, including a series of model updates and fusing models with different modalities.
    
    % \item To overcome the problem of increasing computational cost and storage of the naive solution, we introduce a novel method of a trainable change of basis with extra information to achieve both backward compatibility and not hurting new model by distilling different models into different layers of the distilled model and assembling them by trainable changes of basis.
    % \item We support our framework with strong empirical evidence of guaranteeing backward compatibility while minimally hurting the new model, stably outperforming other state-of-the-art methods with a large margin.
\end{enumerate}

==> CVPR_submission/methodology.tex <==
\section{Methodology}
Our methodology of strategically exploring extra dimensions is mostly inspired by the upper bound solution in the introduction that gets over the trade-off between $\phi_{new}/\phi_{new}$ and $\phi_{old}/\phi_{old}$. We are aware of the two significant drawback of this upper bound solution: 1) it doubles the computations by two forward passes from two models 2) it doubles the dimension of the new representation by naively concatenating $\phi_{old}'$ and $\phi_{new}'$. Our methodology aims to inherit the good theoretical property of the upper bound solution while at the same time minimizing these two drawbacks. In the Subsections \ref{sec:problem setup}, \ref{sec:tradeoff}, and \ref{sec:change of basis}, we introduce some background information for our methodology, while in Subsection \ref{sec:distill} and \ref{sec:merge}, we explain how the two drawbacks of the upper bound solution respectively inspire our design of the model and algorithm.
\subsection{Problem Setup}
\label{sec:problem setup}
We're interested in the following problem setup: given an old representation model that has been trained produces some reasonably good representations $\phi_{old}$, we would like to train a better representation model $\phi_{new}$ with more data or better model architecture. The goal is to achieve the best model possible (for the data and model architecture) while respecting the following commonly accepted criterion for backward compatible representations \cite{9156906, DBLP:journals/corr/abs-2008-04821} is that: 
\begin{definition}[Backward Compatibility]
{ $\phi_{new}$ is backward compatible with $\phi_{old}$, if $\forall x_i, x_j$ from the distribution with interest
\begin{align*} 
    d(\phi_{new}(x_i), \phi_{old}(x_j)) \ge d(\phi_{old}(x_i), \phi_{old}(x_j)), \forall y_i \ne y_j\\ \stepcounter{equation}\tag{\theequation}\label{standard criterion},
    d(\phi_{new}(x_i), \phi_{old}(x_j)) \le d(\phi_{old}(x_i), \phi_{old}(x_j)), \forall y_i = y_j.
\end{align*}
where d is a distance measure, and $(x_i, y_i), (x_j, y_j)$ are samples drawn from the distribution with interest with $x_i, x_j$ being the feature and $y_i, y_j$.
\label{backward compatibility}
}
\end{definition}

Or alternatively, to relax the above criterion because if force constraints on every data point, if there is some empirical metrics $M(\phi^1, \phi^2)$ (for example, top1 accuracy for $\phi^1/\phi^2$), we consider backward compatibility as $M(\phi_{new}, \phi_{old}) >= M(\phi_{old}, \phi_{old})$ .
 
 In addition to the property of backward compatibility, another key property that we're interested in is not hurting the new model:
 
 \begin{definition}[Not Hurting New Model] \label{no hurt}
 Let $\phi_{new}$ be the new embedding model outputted by some compatible training algorithm and $\phi_{new}'$ is an independently trained model with an improved quality over the old model. $\phi_{new}$ is said to be not hurting the new model if, $\forall x_i, x_j$ from the distribution with interest:
 \begin{align*}
    d(\phi_{new}(x_i), \phi_{new}(x_j)) = d(\phi_{new}'(x_i), \phi_{new}'(x_j)) .
\end{align*}
 \end{definition}

Or similarly, if we relax it with an empirical metric $M$, it is turned into $M(\phi_{new}, \phi_{new}) >= M(\phi_{new}', \phi_{new}')$.
 
 In this paper, we adopt the distance metric as the negative dot product for simplicity, but similar conclusion can also be drawn using Euclidean distance as the distance metric:
\begin{align*}
    d(a,b) = - a^\top b
\end{align*}
Note that in this paper, all final representations are normalized, so this dot product is equivalent to cosine similarity.

\subsection{Inherent Trade-off between Backward Compatibility and Not Hurting the New Model}
\label{sec:tradeoff}
We argue that it is required to add new dimensions to the old representation space when necessary, to reliably guarantee backward compatibility and not hurting the new model, and this idea is formalized in Lemma \ref{counterexample}. Intuitively, if the old representation is not good enough and occupies the entire representation space, it leaves no room for possible improvement of the new model in the representation space, that is $\phi_{new}/\phi_{old}$ and $\phi_{new}/\phi_{new}$ cannot be simultaneously achieved.

\begin{lemma} \label{counterexample}
There exists cases where backward compatibility and not hurting the new model cannot be achieved simultaneously without expanding the dimension of the feature space.
\end{lemma}

% \subsection{A Naive Solution to Get Over the Tradeoff}
% In this section, we would like to give a detailed explanation to the naive solution mentioned in the introduction. To ensure that we do not suffer from the tradeoff between $\phi_{new}/\phi_{new}$ and $\phi_{old}/\phi_{old}$, we would like to train two separate models with the new data or model architecture $\phi_{old}'$ to maximize $\phi_{old}'/\phi_{old}$ only and $\phi_{new}'$ to maximize $\phi_{new}'/\phi_{new'}$. Since there is not tradeoff involved in the training of $\phi_{new}'$ and $\phi_{old}'$, both of the two models realize their fullest potential. To get the final new representation $\phi_{new}$, we set \begin{align*}
%     \phi_{new} = \begin{bmatrix}
% \phi_{old}'  \\
% c \times \phi_{new}'  
% \end{bmatrix},
% \end{align*}
% where $c$ is an arbitrary constant. 

\subsection{Learnable Change of Basis for Safe Information Transfer}
\label{sec:change of basis}
In our methodology, we make heavy use of the tool of learnable change of basis. A learnable change of basis $P$ is an orthonormal matrix of dimension $m\times m$, which can be parameterized as the exponential of a left skew-symmetric $A$, so that $P = e^A$, where the upper entries in A are learnable parameters. This design is made possible by the following Lemma~\ref{lemma:matrix exponentiation}
\begin{lemma}
\label{lemma:matrix exponentiation}
    If $A$ is a left skew-symmetric matrix, $P = e^A$ is orthonormal where $P = e^A$ is defined as:
    \begin{align*}
        P = e^A = \sum_{k = 0}^{\infty} \frac{A^k}{k!}
    \end{align*}
\end{lemma}

Intuitively, for any representation $\phi(x)$, applying a change of basis on $\phi(x)$ to get $P\phi(x)$ should not lose any information and will not hurt the quality of the $\phi$. This intuition can be formalized by the following Lemma~\ref{lemma:change of basis}.

\begin{lemma}
\label{lemma:change of basis}
    If $P$ is an orthonormal matrix of dimension $m \times m$, $\forall \phi(x_1), \phi(x_2)$ that are $m$ dimensional vectors:
    \begin{align*}
        \phi(x_1)^\top \phi(x_2) = (P\phi(x_1))^\top (P(\phi(x_2))
    \end{align*}
\end{lemma}

\subsection{Distilling $\phi_{new}'$ and $\phi_{old}'$ into One Model}
\label{sec:distill}
As has been discussed in the introduction \ref{sec:intro}, two major concerns of the upper bound solution are that 1) it requires two models to separately compute $\phi_{new}'$ and $\phi_{old}'$ and 2) it greatly increases the dimension of $\phi_{new}$. In order to solve the first concern, we would like to get both $\phi_{new}'$ and $\phi_{old}'$ from one forward pass. Therefore, we consider the simple solution of a projection layer as illustrated in Figure\ref{projection_layer}, where we train a new backbone with the loss to train $\phi_{new}'$ (classification loss for example) and the loss to train $\phi_{old}'$ (influence loss, for example) applied separately on different layers following the backbone. Concretely, suppose the dimension of $\phi_{new'}$ is $m$ and the dimension of $\phi_{old}'$ is $n$. The new backbone outputs a feature vector with dimension $m+n$ on the first layer where the first $m$ dimensions are trained to mimic $\phi_{new}'$ while the remaining $n$ dimensions are meant to contain some side information for $\phi_{old}'$. Empirically, instead of directly using the remaining $n$ dimensions in the first layer to mimic $\phi_{old}'$, we found that it is better to apply a projection layer that maps all the $m+n$ dimensions in the first layer to an $n$ dimensional vector in the second layer, where it is trained to mimic the $\phi_{old}'$. In this way, we are able to have different layers of our model to mimic $\phi_{new}'$ and $\phi_{old}'$, so that we can get both of the representations with only one forward pass through. We note that compared with the huge backbone, the computation of a projection layer is negligible.

% This section details our solution to the first concern, while the next section shall detail our full methodology as a solution to the second concern as well.



\begin{figure}[!ht]
  \centering
   \includegraphics[width=\linewidth]{projection_layer.pdf}

   \caption{An illustration of our use of projection layer to distill $\phi_{new}'$ and $\phi_{old}'$ into one model.}
   \label{projection_layer}
\end{figure}


\subsection{Merging $\phi_{new}'$ and $\phi_{old}'$ by Learnable Change of Basis}
\label{sec:merge}
In order to solve the second concern, we would like to minimize the use of dimension orthogonal to the old representation. We notice that although new and old models might differ in their model architecture or training data, they should still encode a lot of information in common. Therefore, we propose to train the model to automatically pick out the information of the new representation that is not compatible with the old representation, and only put such extra information on the dimension orthogonal to the old representation. We also want to add additional constraints that in this process, it should not hurt the $\phi_{new}/\phi_{new}$ or $\phi_{new}/\phi_{old}$. It turns out that this constraint can be realized by restricting ourselves by using only learnable change of basis, thanks to the information-preserving property detailed in Lemma \ref{lemma:change of basis}.

\label{learnable basis algorithm}
\begin{algorithm}[t]
\begin{algorithmic} 
\caption{Dimension Reduction by Learnable Change of Basis}
\REQUIRE Learnable backbone $F$ with output dimension $m+n$, learnable projection layer $f$ mapping from dimension $m+n$ to $n+d - m$, learnable change of basis $P_1$ of $m \times m$ and $P_2$ of $n \times $, learnable constant $z < 1$. Constant C and image x.
\STATE $\phi^1 \gets F(x)$
\STATE $\phi^2 \gets f(\phi^1)$, $\phi^2 \gets \frac{\phi^2}{\|\phi^2\|}$
\STATE $\phi^3 \gets \frac{\phi^1[:m]}{\|\phi^1[:m]\|}$
\STATE $\phi^4 \gets C P_1 \phi^1$
\STATE $\phi^5 \gets P_2 \begin{bmatrix} \begin{matrix} &\phi^2 \\ &\phi^3[:m-d]
\end{matrix} \end{bmatrix}$
\STATE $\phi_{new} \gets \begin{bmatrix} \begin{matrix} &\phi^5 \\ &\phi^4[m-d:]
\end{matrix} \end{bmatrix}$
% \STATE \Return $\phi_{new}$
\end{algorithmic}
\end{algorithm}

Figure \ref{dimension_reduction} and Algorithm \ref{learnable basis algorithm} detailed our method to automatically picks out the information in the new representation that is not compatible with the old representation. Compared to Figure \ref{projection_layer}, we mainly add two learnable change of basis to enable the model to automatically pick out the information in the new representation that is incompatible with the old representation, and only put them on the orthogonal dimension of the old representation. Concretely, suppose $\phi_{new}', \phi_{old}'$ are of dimension $m,n$ respectively, and we allow a dimension expansion of $d$, so final embedding of dimension $m+d$,in our budget, our new backbone produces $\phi^1$ of dimension $m+n$ similar to Section \ref{sec:distill} and the first $m$ dimension is trained to mimic $\phi_{new}'$ with the same loss that is used to train $\phi_{new}'$. However, when passing the entire $\phi^1$ into the projection layer, we only produce a $\phi^2$ of dimension $n+d - m$. To pass in the remaining $m-d$ dimension information for $\phi_{old}'$ with information from $\phi_{new}'$, we train two consecutive change of basis layers. First, the first $m$ dimension of $\phi^1$ is passed into the first change of basis $P_1$ to get $\phi^4$, where the first $m-d$ dimension is concatenated with $\phi^2$ and passed into the second change of basis $P_2$ to mix the information of $\phi^2$ and from $\phi^2$ to get $\phi^5$. $\phi^5$ is trained to mimic $\phi_{old}'$ and concatenated with the remaining $d$ dimension of $\phi^4$ to get the final $\phi_{new}$ of dimension $m+d$. Algorithm \ref{learnable basis algorithm} further elaborates some normalization details to ensure the information of $\phi_{new}'$ dominates the information of $\phi_{old}'$ in the final representation $\phi_{new}$.

Despite the technical details in our algorithm, we would like to explain the straightforward main intuition in our algorithm design. We mimic $\phi_{new}'$ and $\phi_{old}'$ indirectly in different layers of our model to minimize the inherent trade-off between $\phi_{new}/\phi_{new}$ and $\phi_{new}/\phi_{old}$, so that we can hope $\phi^3$ learns the best representation for $\phi_{new}/\phi_{new}$ while $\phi^5$ learns the best representation for $\phi_{new}/\phi_{old}$. Since $\phi^5$ is the first $n$ dimension of the final representation $\phi_{new}$, $\phi_{new}$ maintains the same performance of $\phi_{new}/\phi_{old}$ as $\phi^5$. On the other hand, since the information of $\phi^3$ is not lost by the transformation only in the form of change of basis, they all pass to the final $\phi_{new}$ and it is dominant compared to other information in $\phi_{old}'$. By Lemma \ref{lemma:change of basis} and a similar analysis as the upper bound solution, $\phi_{new}$ also attains the best performance of $\phi_{new}/\phi_{new}$ from $\phi^5$. Therefore, our methodology shares a similar theoretical property with the upper bound solution, while significantly the concern of doubling the computations and storage. As we shall see in the experiments, such a principled way of introducing dimensions not only enable us to lead other state-of-the-art methods in the traditional settings, but also enable us to generalize to more practical and useful settings.

==> CVPR_submission/related_works.tex <==
\section{Related Works}
\subsection{Model Compatibility and Backward Compatibility}
Model compatibility has been an increasing focus of research due to its practical significance \cite{DBLP:journals/corr/abs-2108-01958, DBLP:journals/corr/abs-2008-04821, 8953998, https://doi.org/10.48550/arxiv.2107.01057}, where the goal is to contrive a shared representation space where representations from different models can be directly compared. In particular, backward compatibility has been proposed by \cite{9156906} and addressed with an auxilliary loss of influence function. Following works either introduce a transformation module \cite{Hu_2022, ramanujan2022forward, DBLP:journals/corr/abs-2008-04821} or enhanced regularization loss functions \cite{DBLP:journals/corr/abs-2108-01958, DBLP:journals/corr/abs-2201-09724, https://doi.org/10.48550/arxiv.2203.01583}. However, all of the existing approaches fall into one of the following disadvantages: (1) an auxilliary loss prevents the new model to exploit to its fullest potential, (2) a lightweight backfilling is still necessary, and (3) they fail to provide a reliable guarantee of backward compatibility such that backward compatible representation learning may fail in large distribution shift or change in model architecture. In contrast, in this work, we aim to provide reliable backward compatibility without hurting the new model and without requiring any form of backfilling.

\subsection{Continual Learning and Transfer Learning}$\phi_{new}'$ and $\phi_{old}'$
The field of backward compatible representation learning also has a close connection with continual learning \cite{Delange_2021, https://doi.org/10.48550/arxiv.1611.06194, DBLP:journals/corr/abs-1812-00420, DBLP:journals/corr/RebuffiKL16, DBLP:journals/corr/abs-1905-11614} and transfer learning \cite{DBLP:journals/corr/abs-1911-02685, DBLP:journals/corr/ZhangY17aa, 5288526, Zhao2010OTLAF, LU201514}. However, these two fields have a different focus with backward compatible representation learning. Continual learning focuses on training a model to perform well on a new task without forgetting on the old task, and transfer learning focuses on transferring a model to perform well on a different domain with the original training domain. On the other hand, backward compatible representation learning focuses on the same task, i.e. representation learning, such that the representation from the improved new model can be directly used to compare with the old model. 
